Graph Canvas for Controllable 3D Scene Generation

Spatial intelligence is foundational to AI systems that interact with the physical world, particularly in 3D scene generation and spatial comprehension. Current methodologies for 3D scene generation often rely heavily on predefined datasets, and struggle to adapt dynamically to changing spatial relationships. In this paper, we introduce GraphCanvas3D, a programmable, extensible, and adaptable framework for controllable 3D scene generation. Leveraging in-context learning, GraphCanvas3D enables dynamic adaptability without the need for retraining, supporting flexible and customizable scene creation. Our framework employs hierarchical, graph-driven scene descriptions, representing spatial elements as graph nodes and establishing coherent relationships among objects in 3D environments. Unlike conventional approaches, which are constrained in adaptability and often require predefined input masks or retraining for modifications, GraphCanvas3D allows for seamless object manipulation and scene adjustments on the fly. Additionally, GraphCanvas3D supports 4D scene generation, incorporating temporal dynamics to model changes over time. Experimental results and user studies demonstrate that GraphCanvas3D enhances usability, flexibility, and adaptability for scene generation. Our code and models are available on the project website: https://github.com/ILGLJ/Graph-Canvas.

==> sec/Method.tex <==
\section{Method}
\label{sec:Method}




% Text对应物体，Fx。物体与物体的关系（公式），距离（公式）。Pipeline是优化这些东西的。我们是hirerachical的，所以有个Fx = Gx + ...等。

\subsection{Overview}

We present a hirerachical programmable 3D layout paradigm without any pre-defined object information, like using another file to determine the object size and location in this 3D scene. We format the objects, connections in the scene with parameters and functions. Our method can use a single scene description sentence to generate a reasonable scene layout and further render a high quality scene. And for an already rendered scene with our layout paradigm, we can additionally change the layout (like adding a new object to automatically fit the layout or delete a object).

The core of our method is we use a programmable graph structure to organise the layout. From the bottom to top, we define a single object as $o$, the connection between two objects is $l = \zeta(o_i, o_j)$ with an edge-level optimization function $\zeta$. We construct nodes $\mathcal{V} = \{ o_1, \dots, o_N \}$ and edges $\mathcal{E} = \{ l_1, \dots, l_M \}$. For more robust consideration, we first construct several subgraphs with connected nodes to format $G_i = F_s(\mathcal{V_i}, \mathcal{E_i})$, where $F_s$ is the subgraph-level optimzation function. And finally we can use These subgraphs to construct our final graph $\mathcal{G} = F_g(\{G\})$ with the global optimization function $F_g$. 



\subsection{Details} % rewrite it use formula

Given a short scene prompt, we firstly use LLM to analyse the objects and the hidden interactions within those objects with a prompt paradigm. We use a graph to make this layout programmable with those objects to be the nodes of this graph and the interactions to be the edges of this graph. After this transaction, the problem 'set the layout of the scene' changes into modifying the node's location and scale in this scene. 

% Use Point-E to get point clouds
To make the entire layout generation programmable, we use a text-to-3D Generative model like point-e to generate every node's corresponding 3D point clouds. Most of the text-to-3D models's generate result contains no scale information, for example, the point-e can only provide an object with -0.5 to 0.5 in three-axis size range, which is unrealistic when placing two different scale objects together (like a lamp and a table). 

%  Use LLM to infer the possible real scale
However, this can be easily solved when we ask LLM the possible real scale of each object, like LLM can tell "the scale of lamp is 40 cm in width, 40 cm in length and 90 cm in height". Through comparing the size difference between two objects, we can get a premier relative scale ratio between each objects. 

% Explaination of the problem of directly tell place
Current Point clouds understanding models are focusing on understanding the sturcture or details of a single object. It is inadequent to analysis multiply objects' location or distance in a scene. But however current MLLM models shows powerful abilities in image understanding, so we design a four-view rendering methods to help an MLLM to understand a 3D scene.

% Capture the Scene, we find MLLM will give a bad result when directly ask for location
We choose to render an image of a scene in four views: front view, left view, top view, and a view looking at the scene from an angle. Through those views, the MLLM can tell the location of such object in this scene. At first, we want to allow MLLM to directly give an appropriate location of the object, but we found MLLM is weak at determine the location when you want a specific location value of the object. However, when asking a compare relationship of the incorrect object comparing with another object, MLLM can give a reasonable result. We guess this is because the MLLM's the prompt in image understanding training dataset is described in relative position, not the absolution location.

% How to optimise two object
We use MLLM to iterative optimise two objects location in the following steps: 

1. we capture the four-view image of these two objects and use a template prompt to ask MLLM whether the relative scale and location is appropriate. In particular, we will let MLLM to give four score between -100 and 100, to judge whether the scale and location is reasonable comparing to another object.

% ↓ how to describe better? 
% when the incorrect object is too big, give a high score close to 100, when it is too small, give a low score close to -100, when it is at an appropriate scale, give a score nearby 0. And check the three dimensional when the incorrect object is too close to another object, give 

2. We use a loss function the map the provided score into a loss value. This loss function can change the score into a small scale ratio and movement heading the incorrect object to the real layout.

3. We use the scale ratio and movement to optimize the object, and we go back to step 1 for interactively optimization.

% How to construct a subgraph

Through optimising the edge in our graph structure with MLLM, we have already determined an object attributes when it is connected to another object. Thus means when we view these objects in a scene perspective, we will find that if these objects and edges connect each other to form a subgraph, the objects in subgraph are well-placed. So, in the next step we need to place those subgraphs into correct location. We use a prompt to tell the LLM how many objects are in this subgraph and those objects' interaction, size and location. LLM can directly tell us the location of this subgraph is.

% How to modify the current scene
With the organisation with our graph, when there are some scene modification requirements occurs, we can simply change the graph to achieve it. Give a simple requirement which LLM can understand, we can add/delete/move an object. For the most complicated situation like adding an object, the LLM can directly analysis the connection to an occupied node, converting it into an edge structure. With the optimisation of this edge, our structure can automatically spread to the optimisation of the subgraph and graph. The object deleting and moving is much easier.



% from prompt to 3D Gaussian Splatiting
We use MLLM automatically construct a scene using point clouds, however, point clouds are not efficient for high quality rendering and novel view synthesis. For every object in our scene, we can 3DGS for further detailed rendering. 

% MVDream for object
We use MVDream to render every object, ...

% ControlNet for scene
We use ControlNet and SDV1.5 to render the whole scene, making the scene into a unified style.



% For example, the x-axis movement in front view and top view are the 

% We use nodes to present the objects is the basic element of the graph Then we use 3D Generative models like point-e to generate this object's 3D point clouds. 

% Specifically, we utilise a w 


==> sec/backup/3_methods.tex <==


\section{Method}
\label{sec:Method}

\subsection{Problem Formulation}
% Upon receiving a scene prompt, we utilize a large language model (LLM) to parse the prompt and identify the objects present as well as infer any implicit spatial relationships. Each object $o_i$ identified is associated with attributes, such as its type, position, and scale, which are represented as feature vectors $\mathbf{f}_i = [x_i, y_i, z_i, s_i, r_i]$, where $(x_i, y_i, z_i)$ defines the position in 3D space, $s_i$ represents the scale factor \textcolor{red}{ and $r_i$  is the rotation factor along the z-axis. }

% The scene layout generation problem can be mathematically formulated as an optimization problem over the graph $\mathcal{G}$, with the goal of minimizing a global energy function $E_{global}$. The energy function $E_{global}$ is defined as follows:

% \begin{equation}
% E_{global} = F_g(\{ E_{subgraph}(G_i) \}_{i=1}^K),
% \end{equation}

% where $E_{subgraph}(G_i)$ is the energy of a subgraph $G_i$, quantifying the coherence between nodes (objects) and edges (relationships) within that subgraph:

% \begin{equation}
% E_{subgraph}(G_i) = \sum_{(o_p, o_q) \in \mathcal{E}_i} \zeta(o_p, o_q) + \sum_{o_r \in \mathcal{V}_i} \phi(o_r),
% \end{equation}

% where $\zeta(o_p, o_q)$ represents the cost associated with the relationship between objects $o_p$ and $o_q$, and $\phi(o_r)$ is a penalty function that ensures each object $o_r$ adheres to its desired spatial properties, such as alignment, scaling, or position constraints.

% The optimization problem can thus be expressed as:

% \begin{equation}
% \mathcal{G}^* = \arg \min_{\mathcal{G}} E_{global},
% \end{equation}

% where $\mathcal{G}^*$ denotes the optimal graph configuration that yields a coherent scene layout.

In GraphCanvas3D, given a scene prompt, we employ a large language model (LLM) to parse the input, identify objects, and infer both explicit and implicit spatial relationships. Each identified object \( o_i \) is represented by a feature vector \( \mathbf{f}_i \) with components encoding its spatial and geometric attributes:

\[
\mathbf{f}_i = [x_i, y_i, z_i, s_i, r_i],
\]

where:
\begin{itemize}
    \item \( (x_i, y_i, z_i) \) represents the object's 3D spatial position,
    \item \( s_i \) denotes the scale factor, and
    \item \( r_i \) is the rotation factor along the z-axis, an essential attribute for orientational consistency and scene coherence.
\end{itemize}

We frame the 3D scene generation task as an optimization problem over a structured graph \( \mathcal{G} \), where:
\begin{enumerate}
    \item \textbf{Nodes} represent individual objects in the scene, each characterized by a feature vector \( \mathbf{f}_i \) that captures its 3D properties,
    \item \textbf{Edges} denote spatial relationships between objects, derived from linguistic and contextual cues in the scene prompt.
\end{enumerate}

Our objective is to determine an optimal graph configuration \( \mathcal{G}^* \) that reconstructs the 3D scene in alignment with human spatial intuition. This is achieved by minimizing a global energy function \( E_{\text{scene}} \), defined as follows:

\begin{equation}
\mathcal{G}^* = \arg \min_{\mathcal{G}} E_{\text{scene}},
\end{equation}

where \( E_{\text{scene}} \) quantifies deviations from the desired spatial configurations and relationships as inferred from the input prompt.

\subsection{Overview}
As shown in Fig~\ref{fig:pipeline}, We propose a hierarchical, programmable paradigm for 3D layout generation that circumvents the need for predefined object specifications, such as external files containing object dimensions or positions within the 3D scene. Instead, our approach enGraphs object attributes and their interrelationships through a series of parameterized functions. This paradigm facilitates the generation of coherent 3D scene layouts from succinct textual descriptions, followed by high-quality rendering. Furthermore, our layout paradigm supports iterative modifications of previously rendered scenes, enabling users to add new objects that automatically integrate into the existing layout, or to seamlessly remove or reposition elements without disrupting scene coherence.

The core of our methodology centers on a programmable graph that orchestrates the scene layout. Individual objects are represented as nodes, denoted by $o_i$, and spatial relationships between objects are defined as edges, represented by $l_{ij} = \zeta(o_i, o_j)$, where $\zeta$ is an edge-level optimization function that enGraphs the relationship between objects $o_i$ and $o_j$. We formalize the graph as $\mathcal{G} = (\mathcal{V}, \mathcal{E})$, where $\mathcal{V} = \{ o_1, o_2, \dots, o_N \}$ represents the set of nodes, and $\mathcal{E} = \{ l_1, l_2, \dots, l_M \}$ denotes the set of edges connecting these nodes. 

To enhance robustness, we first construct a collection of subgraphs, each consisting of a set of connected nodes, denoted by $G_i = F_s(\mathcal{V}_i, \mathcal{E}_i)$, where $F_s$ is the subgraph-level optimization function that ensures local consistency. These subgraphs are subsequently aggregated to form the complete graph $\mathcal{G} = F_g(\{G_i\})$, with $F_g$ representing the global optimization function responsible for ensuring overall coherence.

\begin{figure*}[ht]
   \centering
   \includegraphics[width=\linewidth]{fig/GraphCanvas3D-EdgeOptim.pdf}
   \caption{\textbf{Edge Optimization Process. }When optimizing an edge, we capture the 3D scene from four different viewpoints to obtain images from these perspectives. These four images are then sent along with an optimized prompt into the MLLMs, which analyzes the inherent relationships between objects across the images and provides corresponding scores. These scores serve as references for optimizing this edge. After passing through activation functions, the scores are propagated to the scene, guiding iterative optimization. }
   \label{fig:edge-optim}
 \end{figure*}

\subsection{Edge-Level Optimization}

To refine the spatial positioning of connected objects, we adopt an iterative optimization approach focusing on edge-level relationships. As shown in Figure ~\ref{fig:edge-optim}, for each pair of connected objects $(o_i, o_j)$, we consider the edge cost $\zeta(o_i, o_j)$, which is dependent on their relative positioning, scaling and rotating. The goal is to minimize discrepancies between the current configuration and the ideal relative positioning derived from high-level scene semantics.

The iterative optimization proceeds as follows:

\begin{enumerate}
    \item Render four distinct views of the subgraph containing the two target objects: front, left, top, and an oblique perspective view. These views are used to generate visual cues for the multimodal LLM.
    
    \item Query the LLM with our predefined edge prompt, assessing whether the current relative positioning and scale are appropriate. The LLM returns a set of scores $\mathbf{s}_{ij} = [s_{ij}^1, s_{ij}^2, s_{ij}^3, s_{ij}^4, s_{ij}^5]$, where $s_{ij}^k \in [-100, 100]$ for $k=1, \dots, 5$, representing the adequacy of the relative arrangement across different views.
    \textcolor{red}{3. Transfer the scores into loss $L_{ij}$. The five generated scores clearly indicate the current optimization direction of the edges. We have set three different activation functions for scale, translation, and rotation. The loss values obtained from these activation functions are directly propagated to the edge structure, guiding the edge optimization process.}
    % 这里要么用上面这个说法，要么就是把Loss值说成是一个vector，一个矢量梯度。还有得加上激活函数
    \item Compute the loss $L_{ij}$ for the edge $l_{ij}$ using a weighted sum of the scores provided by the LLM:
    \begin{equation}
    L_{ij} = \sum_{k=1}^5 w_k \cdot f(s_{ij}^k),
    \end{equation}
    
    where $w_k$ are the weights assigned to each view, and $f(s_{ij}^k)$ is a loss function that penalizes large deviations from the desired spatial relationships.
    
    \item Update the positions and scales of $o_i$ and $o_j$ using a gradient descent step to minimize $L_{ij}$:
\textcolor{red}{When performing edge optimization, we only optimize the incoming vertices to ensure the simplicity of the algorithm.}
    % 这里其实没有优化o_j，只优化o_i
    \begin{equation}
    \mathbf{f}_i \leftarrow \mathbf{f}_i - \eta \frac{\partial L_{ij}}{\partial \mathbf{f}_i}, \quad \mathbf{f}_j \leftarrow \mathbf{f}_j - \eta \frac{\partial L_{ij}}{\partial \mathbf{f}_j},
    \end{equation}
    
    where $\eta$ is the learning rate.

    \item Repeat the process until the loss $L_{ij}$ converges below a predefined threshold.
\end{enumerate}

\textcolor{red}{Since we use a graph structure to manage our scene, all adjacent vertices can be found through edge lookup. By optimizing the incoming vertices in the edges, the corresponding adjacent vertices are also optimized simultaneously. Thus, adjusting only the incoming vertices in edge optimization ensures that the relative positional relationships among other vertices in the graph remain unchanged.
}

\subsection{Subgraph Construction}
Once edge-level optimizations have established robust spatial relationships between connected objects, the next step involves assembling subgraphs into a coherent global scene. Each subgraph $G_i$ is optimized independently to ensure internal coherence. Subsequently, a higher-level optimization function $F_g$ is employed to determine the optimal placement of these subgraphs within the entire scene, ensuring that spatial relationships between different subgraphs are consistent with the overall scene semantics.

The placement of subgraphs is guided by prompts provided to the LLM, which include descriptions of the number of constituent objects, their interrelationships, and inferred sizes. The global optimization objective is thus defined as:

\begin{equation}
\mathcal{G}^* = \arg \min_{\mathcal{G}} \sum_{i=1}^K E_{subgraph}(G_i) + \sum_{(G_p, G_q) \in \mathcal{E}_g} \psi(G_p, G_q),
\end{equation}

where $\psi(G_p, G_q)$ represents the penalty for misalignment or inappropriate spacing between subgraphs $G_p$ and $G_q$.

\subsection{Scene Modification}
Scene modification tasks are readily addressed through the graph representation. For an addition request, a new object node $o_{new}$ is added to the graph, and its connections to existing nodes are established by defining new edges $l_{new, i}$. These new edges are optimized in a similar fashion as described in the edge-level optimization process.

For removal tasks, the corresponding node and its edges are simply deleted from the graph, and the affected neighboring nodes are re-optimized to ensure that the removal does not adversely impact the coherence of the overall layout. Repositioning involves modifying the attributes $\mathbf{f}_i$ of a given node $o_i$, followed by re-optimization of the affected edges and subgraphs.



\subsection{Overall Process} 

\textcolor{red}{We provide a complete example process of our GraphCanvas3D. Given a simple scene prompt input, we use LLM to interprete the nodes prompts and edges prompts. Then we construct our graph with those attributes. The generated node prompts can help us to use 3D generative models like  to predict the corresponding 3D models. For every edge,  we use our four-view caption method to create images and send images to multi-modal LLM to evaluate five scores, repectively control the in-order node's scale, x/y/z-axis translations and the rotation degree through z-axis. Those scores will send to activate functions to provide losses. We iteratively use this optimization method until it surpass a predefined max iteration number. For the subgraph optimisation, we first use Breadth First Search to calculate the subgraph list and provide each subgraph size and information to LLM, LLM can give a location for each subgraph. We use the relative difference to optimise edge and subgraph, so during the final graph-level optimisation, we use the edge connect relationship and subgraph relationship to optimise all nodes into a unified position and scale space, with keeping correct relative attributes for each object and having a plausible attribute towards the scene.}

\subsection{High-Quality Rendering}

While the multimodal LLM facilitates the construction of an initial scene layout using point clouds, these representations are not optimal for high-fidelity rendering or novel view synthesis. To enhance the visual quality of the scenes, we employ 3D Gaussian Splatting (3DGS) for detailed rendering of individual objects.

Additionally, we utilize MVDream for rendering each object with a high level of detail. To ensure stylistic coherence across the entire scene, we leverage ControlNet in conjunction with Stable Diffusion V1.5, thereby facilitating consistency and visual unity throughout the rendered scene.
